Controlled LLM Decoding via Discrete Auto-regressive Biasing

Controlled text generation allows for enforcing user-defined constraints on large language model outputs, an increasingly important field as LLMs become more prevalent in everyday life. One common approach uses energy-based decoding, which defines a target distribution through an energy function that combines multiple constraints into a weighted average. However, these methods often struggle to balance fluency with constraint satisfaction, even with extensive tuning of the energy function's coefficients. In this paper, we identify that this suboptimal balance arises from sampling in continuous space rather than the natural discrete space of text tokens. To address this, we propose Discrete Auto-regressive Biasing, a controlled decoding algorithm that leverages gradients while operating entirely in the discrete text domain. Specifically, we introduce a new formulation for controlled text generation by defining a joint distribution over the generated sequence and an auxiliary bias sequence. To efficiently sample from this joint distribution, we propose a Langevin-within-Gibbs sampling algorithm using gradient-based discrete MCMC. Our method significantly improves constraint satisfaction while maintaining comparable or better fluency, all with even lower computational costs. We demonstrate the advantages of our controlled decoding method on sentiment control, language detoxification, and keyword-guided generation.

==> Experiments/detoxify_table.tex <==
\begin{table}[h]
\caption{Toxicity Avoidance Generation Quality. DAB achieves the best results in terms of directing generation towards less toxic text, as indicated by the internal classifier score, the average external classifier score, and the toxicity prediction probability. In addition to this, DAB maintains competitive fluency metrics, as measured by the CoLA score, the number of repeated trigrams, and the perplexity. This demonstrates that DAB can be used to detoxify text without degrading generation quality.}
\label{table:detoxify}
\centering

\resizebox{\textwidth}{!}{\begin{tabular}{lcccccccl}\toprule
       & \textbf{Int. Clsf Score} & \textbf{Avg Ext. Score} & \textbf{Toxicity Pred. Prob.} & \textbf{CoLA} & \textbf{REP-3gram} & \textbf{PPL} \\\midrule

MuCOLA & $.098 \pm .002$ & $.158 \pm .001$ & $.076 \pm .002$ & $.691 \pm .002$ & $.006 \pm .001$ & $58.015 \pm .435$  \\
COLD & $.136 \pm .002$ & $.184 \pm .001$ & $.102 \pm .002$ & $.667 \pm .001$ & $.024 \pm .001$ & $38.891 \pm .177$  \\
BOLT & $.065 \pm  .001$ & $.153  + .001$ & $\mathbf{.069 \pm  .002}$ & $\mathbf{.830 \pm .001}$ & $\mathbf{.001 \pm.0001}$ & $\mathbf{25.649 \pm .437}$\\
LM-Steer & - & $.157 \pm .001$ & $.079 \pm .002$ & $.722 \pm .002$ & $.006 \pm .002$ & $52.697 \pm .356$   \\\midrule 
DAB & $\mathbf{.057 \pm  .001}$ & $ \mathbf{.143 \pm .001} $ & $\mathbf{.068 + .002}$ & $.806 \pm .001$ & $\mathbf{.001 \pm .0001}$ & $\mathbf{25.609 \pm .126}$ 
\\\bottomrule
\end{tabular}}
\end{table}

==> Experiments/keywords_table.tex <==
\begin{table}[h]
\caption{Sampling Algorithm performance on Keyword Inclusion task. Our method demonstrates superior topicality, as measured by BertScore. Furthermore, our method outperforms all others in terms of the various fluency metrics we use. This demonstrates DAB's ability to direct the auto-regressive generation towards satisfaction of the keyword constraint without sacrificing fluency.}
\label{table:keywords-gen}
\centering

\resizebox{\textwidth}{!}{\begin{tabular}{lccccccl}\toprule
      & \textbf{BertScore (Precision)} & \textbf{Success Rate} & \textbf{CoLA} & \textbf{REP-3gram} & \textbf{PPL} \\\midrule
MuCOLA  & $.8083 \pm .0004$ & $\mathbf{100\%}$&  $.248 \pm .004$ & $.007 \pm .001$ & $475.301 \pm 30.445$ \\
COLD  & $.8123 \pm .0005$ & $\mathbf{100\%}$ &  $.205 \pm .003$ & $.020 \pm .001$ & $ 241.980 \pm 4.943$   \\
BOLT  & $.8291 \pm .0003$ & $99.1\%$ &  $.705 \pm .006$ & $.005 \pm .005$  & $32.019 \pm 1.593$  \\\midrule
DAB  & $\mathbf{.8303 \pm .0003}$ & $99.0\%$ &  $\mathbf{.726 \pm .005}$ & $\mathbf{.004 \pm .001}$  & $\mathbf{23.424 \pm .317}$ 
\\\bottomrule
\end{tabular}}
\end{table}


==> Experiments/sentiment_table.tex <==
\begin{table}[h]
\caption{Sampling Algorithm performance on Sentiment Control task. We evaluate control towards the target attribute via three different classifiers: the internal classifier used to guide the model, an external classifier trained on the same data as the first; and an external classifier trained on a different dataset but intended for the same task. In all three cases, our proposed method beats all baselines. Furthermore, DAB achieves fluency metrics that are competitive with the most fluent baseline, while the most fluent baseline is not able to match DAB's performance for sentiment control. This demonstrates DAB can more effectively control LLM generation without sacrificing as much fluency.}
\label{table:sentiment-control}
\centering

\resizebox{\textwidth}{!}{\begin{tabular}{lcccccccl}\toprule
       & \textbf{Int. Clsf} & \textbf{Ext. Clsf (Yelp)} & \textbf{Ext. Clsf (SST-2)} &  \textbf{CoLA} &  \textbf{REP-3gram} &  \textbf{PPL} \\\midrule

MuCOLA & $.867 \pm .014$ & $.860 \pm .017$ & $.919 \pm .013$ & $.702 \pm .014$ & $.055 \pm .007$ & $33.589 \pm 2.783$ & \\
COLD & $.698 \pm .019$ & $.520 \pm .025$ & $.670 \pm .023$ & $.648 \pm .013$ & $.061 \pm .006$ & $24.970 \pm .873$ &  \\
BOLT & $.926 \pm .007$ & $.754 \pm .021$ & $.872 \pm .015$ & $\mathbf{.874 \pm .009}$ & $\mathbf{.0006 \pm .0003}$ & $\mathbf{11.365 \pm .271}$ &  \\
LM-Steer & - & $.894 \pm .016$ & $.950 \pm .011$ & $.546 \pm .013$ & $.065 \pm .008$ & $77.374 \pm 4.165$ & \\\midrule 
DAB  & $\mathbf{.995 \pm .001}$ & $\mathbf{.899 \pm .015}$ & $\mathbf{.973 \pm .007}$ & $.860 \pm .009$ & $.001 \pm .001$ & $13.148 \pm .308$ &  
\\\bottomrule
\end{tabular}}
\end{table}
